Combinatorial Methods in Grid based Meshing

This paper describes a novel method of generating hex-dominant meshes using pre-computed optimal subdivisions of the unit cube in a grid-based approach. Our method addresses geometries that are standard in mechanical engineering and often must comply with the restrictions of subtractive manufacturability. A central component of our method is the set of subdivisions we pre-compute with Answer Set Programming. Despite being computationally expensive, we obtain optimal meshes of up to 35 nodes available to our method in a template fashion. The first step in our grid-based method generates a coarse Precursor Mesh for meshing complete parts representing the bar stock. Then, the resulting mesh is generated in a subtractive manner by inserting and fitting the pre-generated subdivisions into the Precursor Mesh. This step guarantees that the elements are of good quality. In the final stage, the mesh nodes are mapped to geometric entities of the target geometry to get an exact match. We demonstrate our method with multiple examples showing the strength of this approach.

==> pictures/results/out.tex <==


\begin{figure*}
    \centering
    \begin{tabular}{cccc}
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/3.png  }&
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/5.png  }&
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/7.png  }&
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/15.png }\\
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/20.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/21.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/23.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/26.png }\\
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/27.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/29.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/30.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/31.png }\\
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/60.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/61.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/63.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/90.png }\\
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/91.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/95.png }& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/125.png}& 
    \includegraphics[width=0.23\textwidth]{pictures/maxSJ/127.png}\\
    \end{tabular}
    \caption{All non-trivial subdivisions of a unit cube maximising the minimal SJ.}
    \label{tab:subdivisons}
\end{figure*}



\begin{table*}
    \centering
    \begin{tabular}{cccc}
\includegraphics[width=0.24\textwidth]{pictures/results/B0.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B2.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B4.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B5.png} \\
B0 & B2 & B4 & B5 \\
\includegraphics[width=0.24\textwidth]{pictures/results/B6.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B7.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B9.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B10.png} \\
B6 & B7 & B9 & B10 \\ 
\includegraphics[width=0.24\textwidth]{pictures/results/B11.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B12.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B14.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B15.png} \\
B11 & B12 & B14 & B15 \\
\includegraphics[width=0.24\textwidth]{pictures/results/B17.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B19.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B21.png} & 
\includegraphics[width=0.24\textwidth]{pictures/results/B42.png} \\
B17 & B19 & B21 & B42 \\
\end{tabular}
    \caption{Results for MAMBO geometries}
    \label{tab:MAMBO_1}
\end{table*}



==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
\bibliographystyle{siam}
\bibliography{p}
